Higgs bundles over P^1 and quiver representations

In this note we prove a new explicit formula for the invariants of moduli spaces of twisted Higgs bundles over P^1 and we relate these invariants to the invariants of moduli spaces of representations of some infinite symmetric quiver. The formula can be easily implemented for computations and it is in agreement with the existing conjectures for the invariants of twisted Higgs bundles over curves. Results of this note were presented in Oberwolfach in May 2014.

==> commands.tex <==
%%%%%Utilities%%%%%
\RequirePackage{amsmath,amssymb,xspace}
\RequirePackage{etoolbox,bbm}
\def\mat#1{\ensuremath{#1}\xspace}
\def\dmat#1#2{\gdef#1{\mat{#2}}}
\def\dmata#1#2{\csdef{#1}{\mat{#2}}}
\def\oper#1{\dmata{#1}{\operatorname{#1}}}
\def\opr#1#2{\dmat#1{\operatorname{#2}}}
\def\DMO{\opr}
\def\redef#1{\csletcs{t@#1}{#1}\dmata{#1}{\csuse{t@#1}}}

%%%%%Letters%%%%%%
\def\defbb#1{\dmata{b#1}{\mathbb{#1}}}%\bA
\def\defcal#1{\dmata{c#1}{\mathcal{#1}}}%\cA
\def\deffrak#1{\dmata{f#1}{\mathfrak{#1}}}%\fA 
\def\defbf#1{\dmata{bf#1}{\mathbf{#1}}}%\bfA
\def\defall#1{\defbb{#1}\defcal{#1}\deffrak{#1}}
\forcsvlist\defall{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}
\forcsvlist\deffrak{a,b,c,d,e,f,g,h,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z}
\RequirePackage{bbm}
\dmat\bk{{\mathbbm{k}}}
\forcsvlist\defbf{E,F,H,L,M}

%%%%%Greek letters%%%%%
\def\do#1{\dmat#1}
\docsvlist{\al\alpha,\be\beta,\ga\gamma,\Ga\Gamma,\de\delta,\De\Delta,\eps\varepsilon,\hi\chi,\kp\kappa,\ksi\xi,\La\Lambda,\la\lambda,\Om\Omega,\om\omega,\vi\varphi,\si\sigma,\Si\Sigma,\ze\zeta,\te\theta,\Te\Theta,\ta\tau}
\forcsvlist\redef{eta,xi,mu,nu,Phi,Psi,psi,pi,rho,Pi}

%%%%%Operators%%%%%
\forcsvlist\oper{Ind,rad,Res,Rep,Sym,Gr,vol}
\forcsvlist\oper{Hom,End,Aut,Ext,GL}
\forcsvlist\oper{Bun,Coh,Spec,Pic,Proj,supp}
\forcsvlist\oper{Exp,Log,Pow,pow}
\forcsvlist\oper{Id,rk,coker,im,tr}
\DMO\cHom{\cH\kern-1.5pt\mathit{om}}
\DMO\SHom{\cS\cH\kern-1.5pt\mathit{om}}
\DMO\lEnd{\cE\kern-2.5pt\mathit{nd}}
\DMO\SEnd{\cS\cE\kern-2.5pt\mathit{nd}}
\def\gl{\mathfrak{gl}}

%%%%%Structures%%%%%
\def\set#1{\mat{\{#1\}}}
\def\sets#1#2{\mat{\left\{\left.#1\vphantom{#2}\,\right\vert#2\right\}}}
\def\rbr#1{\left(#1\right)}
\def\sbr#1{\left[#1\right]}
\def\qbinom#1#2{\mat{\genfrac{[}{]}{0pt}{}{#1}{#2}}}  %q-binomial
\def\ang#1{\mat{\left\langle#1\right\rangle}}
\def\angs#1#2{\mat{\left<\left.#1\vphantom{#2}\,\right\vert#2\right>}}
\def\eq#1{\begin{equation}#1\end{equation}}
\def\eql#1#2{\begin{equation}\label{#2}#1\end{equation}}

%%%%%Symbols%%%%%
\def\n#1{\mat{\left\lvert#1\right\rvert}}
\def\nn#1{\mat{\left\lVert#1\right\rVert}}
\def\lb#1{\mat{\underline{#1}}} %lower bar
\def\ub#1{\mat{\overline{#1}}}  %upper bar
\def\what#1{\mat{\widehat{#1}}}
\def\pser#1{[\![#1]\!]} %formal power series [[#1]]
\def\ov#1#2{{\substack{#1\\#2}}} %#1 over #2
\redef{iff}
\def\mto{\mapsto}
\def\emb{\hookrightarrow}
\dmat\es\varnothing%\emptyset
\def\iso{\simeq}
\def\ts{\otimes}
\def\sbs{\subset}
\def\sps{\supset}
\def\xx{\times}
\def\ms{\backslash} %minus set
\def\partof{\vdash}
\def\bop{\bigoplus}
\def\one{\mathbbm{1}}%\def\one{\mathbf{1}}
\def\dlim{\varinjlim} %direct limit
\dmat\oh{\frac12}
\def\git{/\!\!/}
\dmat\Gm{{\bG_{\mathrm m}}}
\dmat\sst{\mathrm{sst}}
\dmat\st{\mathrm{s}}
\dmat\nil{\mathrm{nil}}
\dmat\gr{\mathrm{gr}}
\def\inv{^{-1}}
\def\lqq{\lq\lq}
\def\rqq{\rq\rq\xspace}
\def\ie{i.e.\ }
\def\eg{e.g.\ }
\def\cf{cf.\ }

%%%%%Theorems%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conjecture}{Conjecture}
\theoremstyle{definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\AtEndEnvironment{example}{\hfill$\lozenge$}
\AtEndEnvironment{remark}{\hfill$\lozenge$}

%%%%%Notes%%%%%
%\RequirePackage{mdframed}
\usepackage[framemethod=TikZ]{mdframed}
\newmdtheoremenv[backgroundcolor=green!25, roundcorner=5pt,skipabove=5pt,innertopmargin=0pt]{notesa}[theorem]{Note}
\newenvironment{notes}{\begin{notesa}}{\end{notesa}}
%\RequirePackage{comment}
%\excludecomment{notes}

\RequirePackage{todonotes}
\def\note#1{\ \todo[inline,bordercolor=green,backgroundcolor=green!25]{#1}} %[disable] option

\def\hr{\makebox[\linewidth]{\rule{\paperwidth}{0.4pt}}\newline}

%%%%%Citations \cite[#1]{#2}[#3]%%%%%
\RequirePackage{xparse}
\csletcs{t@cite}{cite}
\DeclareDocumentCommand{\citeomo}{omo}{%
\IfValueTF{#1}{\csuse{t@cite}[#1]{#2}}%
{\IfValueTF{#3}{\csuse{t@cite}[#3]{#2}}%
{\csuse{t@cite}{#2}}}}
\def\cite{\citeomo}

%%%%%Additional symbols%%%%%
\def\xto{\xrightarrow}
\def\lto{\leftarrow}
\def\xlto{\xleftarrow}
\def\bw{\mathbf w}
\def\p#1{\mat{\mathbf{#1}}} %parabolic
\dmat\pE{\p E}
\dmat\pF{\p F}
\dmat\pG{\p G}
\def\h#1{\mat{\bar{#1}}} %higgs
\def\ph#1{\mat{\mathbf{\bar{#1}}}} %parabolic Higgs
\def\fo#1{\mat{\hat{#1}}} %framed object
\def\fr{\mathsf{fr}}
\opr\Fr{\Pi}
\opr\Higgs{Higgs}
\oper{Reg}
\oper{pardeg}
\opr\udim{\mathbf{dim}}
\def\lft#1{#1^*}
\def\pdeg{\operatorname{deg}_\te}
\def\mut{\mu_\te}
\dmat\cs{\mathfrak{G}} %counting sequences, ghosts

\def\ci{\mathbf{i}}%counting indecomp
\def\ca{\mathbf{a}}%counting abs indecomp
\def\spl{\mathfrak K}%splitting field
\def\mt#1{\bfM^{\te-\sst}_{#1}}%groupoid of \te-semist par higgs bundles
\def\mm#1{\bfM_{#1}}%gropoid of all par higgs bundles

\def\yoko#1{\cite[#1]{yokogawa_infinitesimal}}
\def\ldiv{\operatorname{\mathfrak{Div}}}
\def\lpic{\operatorname{\mathfrak{Pic}}}
\def\wt{\mathrm{wt}}
\def\gp{\mathrm{gp}}

%\Requirepackage{bm}
\def\pHom{\bm{\mathcal Hom}}


%%%%% a22.1
\def\gnil{\mathbf{Nil}}
\def\gcoh{\mathbf{Coh}}
\def\gfil{\mathbf{Filt}}
\def\one{\mathbbm{1}}%{\mathbf{1}}
\def\w{z}
\def\z{w}
\def\hnsp{\si}

\def\higgMod{\mathcal M}
\def\higgInv{\mathsf H}
\def\hb#1#2{\mat{\higgMod_{#1}(#2)}}
\def\hp#1#2{\mat{\higgMod_{#1}^{>0}(#2)}}
\def\hpn#1#2{\mat{\higgMod_{#1,\mathrm{nil}}^{>0}(#2)}}
\def\ihb#1#2{\mat{\mathsf{\higgInv}_{#1}(#2)}}
\def\ihp#1#2{\mat{\higgInv_{#1}^{>0}(#2)}}
\def\ihpn#1#2{\mat{\higgInv_{#1,\mathrm{nil}}^{>0}(#2)}}
\def\cp{\cA^{>0}}%category of sheaves with positive HN factors
\def\chb#1{\cA_D}%category of D-twisted Higgs bundles
\def\chp#1{\cA_D^{>0}}%the same with positive HN factors

%\makeatletter
%\def\to{\@ifnextchar^{\expandafter\xrightarrow\@gobble}\rightarrow}
%\makeatother


\def\h#1{\bar{#1}} %higgs
\def\hE{\h E}
\def\hF{\h F}
\def\cha{\operatorname{ch}}
\dmat\a{\cA}
\def\bul{\bullet}
\def\lInto{\hookleftarrow}
\def\wtl{\widetilde}
\oper{Higgs}
\def\rbb#1{\Bigg(#1\Bigg)}%round bracket, big
\def\lf{\bL^\oh-\bL^{-\oh}}
\def\lfb{\big(\lf\big)}
\def\tpdf#1#2{\texorpdfstring{#1}{#2}}
\def\ma{\cM^{\mathrm a}}%stack of all repres.
\def\vir{\mathrm{vir}}
\def\mot#1{\sbr{#1}}
\def\vmot#1{\sbr{#1}_\vir}



